Generative AI for Synthetic Data Across Multiple Medical Modalities: A Systematic Review of Recent Developments and Challenges

This paper presents a comprehensive systematic review of generative models (GANs, VAEs, DMs, and LLMs) used to synthesize various medical data types, including imaging (dermoscopic, mammographic, ultrasound, CT, MRI, and X-ray), text, time-series, and tabular data (EHR). Unlike previous narrowly focused reviews, our study encompasses a broad array of medical data modalities and explores various generative models. Our search strategy queries databases such as Scopus, PubMed, and ArXiv, focusing on recent works from January 2021 to November 2023, excluding reviews and perspectives. This period emphasizes recent advancements beyond GANs, which have been extensively covered previously. The survey reveals insights from three key aspects: (1) Synthesis applications and purpose of synthesis, (2) generation techniques, and (3) evaluation methods. It highlights clinically valid synthesis applications, demonstrating the potential of synthetic data to tackle diverse clinical requirements. While conditional models incorporating class labels, segmentation masks and image translations are prevalent, there is a gap in utilizing prior clinical knowledge and patient-specific context, suggesting a need for more personalized synthesis approaches and emphasizing the importance of tailoring generative approaches to the unique characteristics of medical data. Additionally, there is a significant gap in using synthetic data beyond augmentation, such as for validation and evaluation of downstream medical AI models. The survey uncovers that the lack of standardized evaluation methodologies tailored to medical images is a barrier to clinical application, underscoring the need for in-depth evaluation approaches, benchmarking, and comparative studies to promote openness and collaboration.

==> 7_acronyms.tex <==
Generative Adversarial Networks (GANs)
Variational Autoencoders (VAEs)
Diffusion Models (DMs)
Large Language Models (LLMs)
Artificial Intelligence (AI)
Machine Learning (ML)
Electronic Health Records (EHR)
Electrocardiography (ECG)
Electroencephalography (EEGs)
Computed Tomography (CT)
Magnetic Resonance Imaging (MRI)
Optical Coherence Tomography (OCT)
Natural Language Processing (NLP)
Name Entity Recognition (NER)
Recurrent Neural Networks (RNNs), 
Gated Recurrent Units (GRUs), 
Long Short-term Memory(LSTMs)
Deep Convolutional GAN (DCGAN)
Wasserstein GAN (WGAN)
Least Squares GAN (LSGAN)
Progressive Growing GAN (PGGAN)
Wasserstein GAN with gradient penalty (WGAN-GP)
Conditional Generative Adversarial Networks (cGANs)
Style Generative Adversarial Network (StyleGAN)
spatially-adaptive (SPADE)
Vector-Quantized Variational Autoencoder (VQ-VAE)8
Vector-Quantized Generative Adversarial Network (VQ-GAN)
vector quantization (VQ)
Diffusion Probabilistic Models (DPMs)
Denoising Diffusion Probabilistic Models (DDPM)
Bidirectional Recurrent Neural Networks (BRNNs)
Latent Diffusion Model (LDM)
Contrastive Language-Image Pre-training (CLIP)
Byte Pair Encoding (BPE)
Self-alignment pretraining for BERT (SAPBERT)
BERT (Bidirectional Encoder Representations from Transformers)
GPT-2 (Generative Pretrained Transformer 2)
Llama (Large Language Model Meta AI) 
FLAN-T5 (Fine-tuned LAnguage Net with a Text-To-Text Transfer Transformer)
Nearest Neighbor Adversarial Accuracy (NNAA)
differential privacy (DP)
FID (Frechet Inception Distance)
IS (Inception Score)
t-distributed Stochastic Neighbor Embedding (t-sne) 
Principal Component Analysis (PCA)
International Classification of Diseases (ICD)
Stochastic Differential Equation (SDE)
Conditional tabular GANs (CTGANs)
Tabular GAN (TGAN)
conditional TableGAN (CTABGAN)
Atrial Fibrillation (AF)
Heart rate variability (HRV)
Structured State Space Model (SSSM)
Convolutional Neural Network (CNN)
Causal Recurrent Variational Autoencoder (CR-VAE)
Class conditional Wasserstein GAN (CWGAN)
Short-time Fourier transform (STFT)
”Unsupervised Data Augmentation for Consistency Training” (UDA)
SyleGAN2 with adaptive discriminator augmentation (StyleGAN2-ADA)
Differentiable Augmentation (DiffAugment)
Digitized Screen-film Mammograms (DFMs)
Full-Field Digital Mammography (FFDM)
digital breast tomosynthesis (DBT)
Pair with Constraint (PWC)
region of interest (ROI)
Brightness mode (B-mode)
Elastography Ultrasound (EUS)
anatomical model (AM)
Transformer-based GAN (TB-GAN)
four-chamber (FC)
intra-operative US (iUS)
Ultrasound (US)
preoperative magnetic resonance (pMR)
Multi-Modal Hierarchical Latent Representation VAE (MHVAE)
anatomy preserving GAN (ApGAN)
intra-operative ultrasound (Sim-iUS)
pre-operative MR (pMR)
Interpretable Representation Learning by Information Maximizing Generative Adversarial Nets (InfoGAN)
Temporal Recurrent GAN (TR-GAN)
context-aware generative adversarial network (CoCa-GAN)
disentangled anatomy arithmetic GAN (DAA-GAN)
low-dose CT (LDCT)
Multi-Condition Diffusion Probabilistic Model (MC-DPM)
Multiple Gradient Descent Algorithm (MGDA)
semantic diffusion models (SDM)
HED (Holistically-Nested Edge Detection)
GAN with Noise Encoding Transfer Learning (GAN-NETL)
normal-dose CT (NDCT)
Cone beam CT (CBCT)
chest X-rays (CXR)
Universal Image Quality Index (UIQI)
Visual Information Fidelity (VIF)
Fourier Attention Block (FAB)
spectral domain OCT (SD-OCT)
fast Fourier transform (FFT)
post-therapeutic (PT)
Adaptive Memory Batch Normalization (AMBN)
age-related macular degeneration (AMD)
neovascular age-related macular degeneration (nAMD)
Kernel Inception Distance (KID)
anti-vascular endothelial growth factors (anti-VEGF)
polarization-sensitive (PS)
fluorescein angiography (FA)
diversity score (DS)
n2c2 (National NLP Clinical Challenges)
History and Present Illness (HPI)
CharRNN(Character Recurrent Neural Network)
SegGAN (Sub-sequence Generative Adversarial Network)
Conditional Transformer Language (CTRL) 
Bilingual Evaluation Understudy (BLEU)
downstream task (DT)
Synthetic ranking agreement (SRA)
Deep convolutional conditional GAN (DCCGAN)
Region-Disentangled Diffusion Model (RDDM)
causal recurrent VAE (CRVAE), temporal GAN (TGAN)
complete representation GAN (CR-GAN)
texture-constrained multichannel progressive GAN (TMP-GAN)
high resolution GAN (HRGAN)
Multi-Modal Hierarchical Latent Representation VAE (MHVAE)
anatomy preserving GAN (ApGAN)
Pseudo-Siamese Feature Fusion Generative Adversarial Network (PSFFGAN)
GAN with coordinate attention mechanism (GAN-CA)
Diffusion-Super-Resolution-GAN (DSR-GAN)
Transformer-based-GAN (TB-GAN)
anterior segment  (AS)
spectral domain  (SD) 
diabetic maculopathy  (DM) 
foveal hypoplasia (FH) 
diabetic macular edema (DME) 
color fundus photography (CFP)
pre-therapy (Pre-T)
post-therapy (Post-T) 


==> acro_list.tex <==
\DeclareAcronym{gan}{
  short=GAN,
  long=Generative Adversarial Network,
}
\DeclareAcronym{vae}{
  short=VAE,
  long=Variational Autoencoder,
}
\DeclareAcronym{dm}{
  short=DM,
  long=Diffusion Model,
}
\DeclareAcronym{llm}{
  short=LLM,
  long=Large Language Model,
}
\DeclareAcronym{ai}{
  short=AI,
  long=Artificial Intelligence,
}
\DeclareAcronym{ml}{
  short=ML,
  long=Machine Learning,
}
\DeclareAcronym{ehr}{
  short=EHR,
  long=Electronic Health Records,
}
\DeclareAcronym{ecg}{
  short=ECG,
  long=Electrocardiography,
}
\DeclareAcronym{eeg}{
  short=EEG,
  long=Electroencephalography,
}
\DeclareAcronym{ct}{
  short=CT,
  long=Computed Tomography,
}
\DeclareAcronym{mri}{
  short=MRI,
  long=Magnetic Resonance Imaging,
}
\DeclareAcronym{oct}{
  short=OCT,
  long=Optical Coherence Tomography,
}
\DeclareAcronym{nlp}{
  short=NLP,
  long=Natural Language Processing,
}
\DeclareAcronym{ner}{
  short=NER,
  long=Name Entity Recognition,
}
\DeclareAcronym{rnn}{
  short=RNN,
  long=Recurrent Neural Network,
}
\DeclareAcronym{gru}{
  short=GRU,
  long=Gated Recurrent Units,
}
\DeclareAcronym{lstm}{
  short=LSTM,
  long=Long Short-term Memory,
}
\DeclareAcronym{dcgan}{
  short=DCGAN,
  long=Deep Convolutional GAN,
}
\DeclareAcronym{wgan}{
  short=WGAN,
  long=Wasserstein GAN,
}
\DeclareAcronym{lsgan}{
  short=LSGAN,
  long=Least Squares GAN,
}
\DeclareAcronym{pggan}{
  short=PGGAN,
  long=Progressive Growing GAN,
}
\DeclareAcronym{wgangp}{
  short=WGAN-GP,
  long=Wasserstein GAN with gradient penalty,
}
\DeclareAcronym{cgan}{
  short=cGAN,
  long=Conditional Generative Adversarial Network,
}
\DeclareAcronym{stylegan}{
  short=StyleGAN,
  long=Style Generative Adversarial Network,
}
\DeclareAcronym{spade}{
  short=SPADE,
  long=spatially-adaptive,
}
\DeclareAcronym{vqvae}{
  short=VQ-VAE,
  long=Vector-Quantized Variational Autoencoder,
}
\DeclareAcronym{vqgan}{
  short=VQ-GAN,
  long=Vector-Quantized Generative Adversarial Network,
}
\DeclareAcronym{vq}{
  short=VQ,
  long=vector quantization,
}
\DeclareAcronym{dpm}{
  short=DPM,
  long=Diffusion Probabilistic Models,
}
\DeclareAcronym{ddpm}{
  short=DDPM,
  long=Denoising Diffusion Probabilistic Models,
}
\DeclareAcronym{brnn}{
  short=BRNN,
  long=Bidirectional Recurrent Neural Networks,
}
\DeclareAcronym{ldm}{
  short=LDM,
  long=Latent Diffusion Model,
}
\DeclareAcronym{clip}{
  short=CLIP,
  long=Contrastive Language-Image Pre-training,
}
\DeclareAcronym{bpe}{
  short=BPE,
  long=Byte Pair Encoding,
}
\DeclareAcronym{sapbert}{
  short=SAPBERT,
  long=Self-alignment pretraining for BERT,
}
\DeclareAcronym{bert}{
  short=BERT,
  long=Bidirectional Encoder Representations from Transformers,
}
\DeclareAcronym{gpt2}{
  short=GPT-2,
  long=Generative Pretrained Transformer 2,
}
\DeclareAcronym{llama}{
  short=Llama,
  long=Large Language Model Meta AI,
}
\DeclareAcronym{flant5}{
  short=FLAN-T5,
  long=Fine-tuned LAnguage Net with a Text-To-Text Transfer Transformer,
}
\DeclareAcronym{nnaa}{
  short=NNAA,
  long=Nearest Neighbor Adversarial Accuracy,
}
\DeclareAcronym{dp}{
  short=DP,
  long=differential privacy,
}
\DeclareAcronym{fid}{
  short=FID,
  long=Frechet Inception Distance,
}
\DeclareAcronym{is}{
  short=IS,
  long=Inception Score,
}
\DeclareAcronym{tsne}{
  short=t-sne,
  long=t-distributed Stochastic Neighbor Embedding,
}
\DeclareAcronym{pca}{
  short=PCA,
  long=Principal Component Analysis,
}
\DeclareAcronym{icd}{
  short=ICD,
  long=International Classification of Diseases,
}
\DeclareAcronym{sde}{
  short=SDE,
  long=Stochastic Differential Equation,
}
\DeclareAcronym{ctgan}{
  short=CTGAN,
  long=Conditional tabular GANs,
}
\DeclareAcronym{tgan}{
  short=TGAN,
  long=Tabular GAN,
}
\DeclareAcronym{ctabgan}{
  short=CTABGAN,
  long=conditional TableGAN,
}
\DeclareAcronym{af}{
  short=AF,
  long=Atrial Fibrillation,
}
\DeclareAcronym{hrv}{
  short=HRV,
  long=Heart rate variability,
}
\DeclareAcronym{sssm}{
  short=SSSM,
  long=Structured State Space Model,
}
\DeclareAcronym{cnn}{
  short=CNN,
  long=Convolutional Neural Network,
}
\DeclareAcronym{crvae}{
  short=CR-VAE,
  long=Causal Recurrent Variational Autoencoder,
}
\DeclareAcronym{cwgan}{
  short=CWGAN,
  long=Class conditional Wasserstein GAN,
}
\DeclareAcronym{stft}{
  short=STFT,
  long=Short-time Fourier transform,
}
\DeclareAcronym{uda}{
  short=UDA,
  long=Unsupervised Data Augmentation for Consistency Training,
}
\DeclareAcronym{stylegan2ada}{
  short=StyleGAN2-ADA,
  long=SyleGAN2 with adaptive discriminator augmentation,
}
\DeclareAcronym{diffaugment}{
  short=DiffAugment,
  long=Differentiable Augmentation,
}
\DeclareAcronym{dfms}{
  short=DFMs,
  long=Digitized Screen-film Mammograms,
}
\DeclareAcronym{ffdm}{
  short=FFDM,
  long=Full-Field Digital Mammography,
}
\DeclareAcronym{dbt}{
  short=DBT,
  long=digital breast tomosynthesis,
}
\DeclareAcronym{pwc}{
  short=PWC,
  long=Pair with Constraint,
}
\DeclareAcronym{roi}{
  short=ROI,
  long=region of interest,
}
\DeclareAcronym{bmode}{
  short=B-mode,
  long=Brightness mode,
}
\DeclareAcronym{tbgan}{
  short=TB-GAN,
  long=Transformer-based GAN,
}
\DeclareAcronym{fc}{
  short=FC,
  long=four-chamber,
}
\DeclareAcronym{ius}{
  short=iUS,
  long=intra-operative US,
}
\DeclareAcronym{us}{
  short=US,
  long=Ultrasound,
}
\DeclareAcronym{pmr}{
  short=pMR,
  long=preoperative magnetic resonance,
}
\DeclareAcronym{mhvae}{
  short=MHVAE,
  long=Multi-Modal Hierarchical Latent Representation VAE,
}
\DeclareAcronym{apgan}{
  short=ApGAN,
  long=anatomy preserving GAN,
}
\DeclareAcronym{simius}{
  short=Sim-iUS,
  long=intra-operative ultrasound,
}
\DeclareAcronym{pmr}{
  short=pMR,
  long=pre-operative MR,
}
\DeclareAcronym{infogan}{
  short=InfoGAN,
  long=Interpretable Representation Learning by Information Maximizing Generative Adversarial Nets,
}
\DeclareAcronym{trgan}{
  short=TR-GAN,
  long=Temporal Recurrent GAN,
}
\DeclareAcronym{cocagan}{
  short=CoCa-GAN,
  long=context-aware generative adversarial network,
}
\DeclareAcronym{daagan}{
  short=DAA-GAN,
  long=disentangled anatomy arithmetic GAN,
}
\DeclareAcronym{ldct}{
  short=LDCT,
  long=low-dose CT,
}
\DeclareAcronym{mcdpm}{
  short=MC-DPM,
  long=Multi-Condition Diffusion Probabilistic Model,
}
\DeclareAcronym{mgda}{
  short=MGDA,
  long=Multiple Gradient Descent Algorithm,
}
\DeclareAcronym{sdm}{
  short=SDM,
  long=semantic diffusion models,
}
\DeclareAcronym{hed}{
  short=HED,
  long=Holistically-Nested Edge Detection,
}
\DeclareAcronym{gannetl}{
  short=GAN-NETL,
  long=GAN with Noise Encoding Transfer Learning,
}
\DeclareAcronym{ndct}{
  short=NDCT,
  long=normal-dose CT,
}
\DeclareAcronym{cbct}{
  short=CBCT,
  long=Cone beam CT,
}
\DeclareAcronym{cxr}{
  short=CXR,
  long=chest X-rays,
}
\DeclareAcronym{uiqi}{
  short=UIQI,
  long=Universal Image Quality Index,
}
\DeclareAcronym{vif}{
  short=VIF,
  long=Visual Information Fidelity,
}
\DeclareAcronym{fab}{
  short=FAB,
  long=Fourier Attention Block,
}
\DeclareAcronym{sd-oct}{
  short=SD-OCT,
  long=spectral domain OCT,
}
\DeclareAcronym{fft}{
  short=FFT,
  long=fast Fourier transform,
}
\DeclareAcronym{pt}{
  short=PT,
  long=post-therapeutic,
}
\DeclareAcronym{ambn}{
  short=AMBN,
  long=Adaptive Memory Batch Normalization,
}
\DeclareAcronym{amd}{
  short=AMD,
  long=age-related macular degeneration,
}
\DeclareAcronym{namd}{
  short=nAMD,
  long=neovascular age-related macular degeneration,
}
\DeclareAcronym{kid}{
  short=KID,
  long=Kernel Inception Distance,
}
\DeclareAcronym{antivegf}{
  short=anti-VEGF,
  long=anti-vascular endothelial growth factors,
}
\DeclareAcronym{ps}{
  short=PS,
  long=polarization-sensitive,
}
\DeclareAcronym{fa}{
  short=FA,
  long=fluorescein angiography,
}
\DeclareAcronym{ds}{
  short=DS,
  long=diversity score,
}
\DeclareAcronym{n2c2}{
  short=n2c2,
  long=National NLP Clinical Challenges,
}
\DeclareAcronym{hpi}{
  short=HPI,
  long=History and Present Illness,
}
\DeclareAcronym{charRNN}{
  short=CharRNN,
  long=Character Recurrent Neural Network,
}
\DeclareAcronym{seggan}{
  short=SegGAN,
  long=Sub-sequence Generative Adversarial Network,
}
\DeclareAcronym{ctrl}{
  short=CTRL,
  long=Conditional Transformer Language,
}
\DeclareAcronym{bleu}{
  short=BLEU,
  long=Bilingual Evaluation Understudy,
}
\DeclareAcronym{dt}{
  short=DT,
  long=downstream task,
}
\DeclareAcronym{sra}{
  short=SRA,
  long=Synthetic ranking agreement,
}
\DeclareAcronym{dccgan}{
  short=DCCGAN,
  long=Deep convolutional conditional GAN,
}
\DeclareAcronym{rddm}{
  short=RDDM,
  long=Region-Disentangled Diffusion Model,
}
\DeclareAcronym{crvae}{
  short=CRVAE,
  long=causal recurrent VAE,
}
\DeclareAcronym{tgan}{
  short=TGAN,
  long=temporal GAN,
}
\DeclareAcronym{cr-gan}{
  short=CR-GAN,
  long=complete representation GAN,
}
\DeclareAcronym{tmp-gan}{
  short=TMP-GAN,
  long=texture-constrained multichannel progressive GAN,
}
\DeclareAcronym{hrgan}{
  short=HRGAN,
  long=high resolution GAN,
}
\DeclareAcronym{mhvae}{
  short=MHVAE,
  long=Multi-Modal Hierarchical Latent Representation VAE,
}
\DeclareAcronym{apgan}{
  short=ApGAN,
  long=anatomy preserving GAN,
}
\DeclareAcronym{psffgan}{
  short=PSFFGAN,
  long=Pseudo-Siamese Feature Fusion Generative Adversarial Network,
}
\DeclareAcronym{gan-ca}{
  short=GAN-CA,
  long=GAN with coordinate attention mechanism,
}
\DeclareAcronym{dsr-gan}{
  short=DSR-GAN,
  long=Diffusion-Super-Resolution-GAN,
}
\DeclareAcronym{tbgan}{
  short=TB-GAN,
  long=Transformer-based GAN,
}
\DeclareAcronym{as}{
  short=AS,
  long=anterior segment,
}
\DeclareAcronym{sd}{
  short=SD,
  long=spectral domain,
}
\DeclareAcronym{dm}{
  short=DM,
  long=diabetic maculopathy,
}
\DeclareAcronym{fh}{
  short=FH,
  long=foveal hypoplasia,
}
\DeclareAcronym{dme}{
  short=DME,
  long=diabetic macular edema,
}
\DeclareAcronym{cfp}{
  short=CFP,
  long=color fundus photography,
}
\DeclareAcronym{pre-t}{
  short=Pre-T,
  long=pre-therapy,
}
\DeclareAcronym{post-t}{
  short=Post-T,
  long=post-therapy,
}


==> discusssion.tex <==



\section{Discussion}
\label{sec:discussion}
% \cite{multi-20} only paper that generate tabular and imaging data together 


% \subsection{Privacy- to be merged with thte below}
% One paper \cite{multi-7} talk about image encryption.Some of the key points of the paper are:

% Motivation: The paper argues that encrypting sensitive information of medical images is a challenging task that requires high computational complexity and robustness against various attacks. The paper reviews the existing methods for image encryption and identifies their limitations, such as high cost, low efficiency, and poor image quality.
% Method: The paper introduces a new framework called DeepGAN, which uses a GAN as a learning network to generate a private key for image encryption. The paper also uses a transformation domain to guide the learning network and preserve the unique features of the private key. The paper describes the details of the DeepGAN architecture, the training process, and the encryption and decryption algorithms.
% Results: The paper evaluates the performance and security of the DeepGAN method on three open-source medical datasets: the Ultrasonic Brachial Plexus, the Montgomery County Chest X-ray, and the BraTS18. The paper compares the DeepGAN method with other image encryption methods and shows that the DeepGAN method achieves higher image quality, lower computational cost, and stronger resistance to various attacks. The paper also shows some examples of the synthesized medical images generated by the DeepGAN method.

% Two papers talk about memorization inn medical imaging:\cite{mutli-4} and \cite{r-175}

% \textbf{From \cite{multi-4}:
% }

% To investigate memorization is even more important for larger models; their diffusion model had 1.6 billion trainable parameters (which is substantially higher compared to the GANs used for comparison). Pinaya et al. \cite{mri-17} also used SSIM to investigate the diversity of the generated brain volumes, but did not calculate SSIM between real and synthetic volumes. 

%todo Packhauser et al. [24] guaranteed patient privacy by using additional networks to remove synthetic images that are too similar to the training images. However, it is not mentioned how many synthetic images that were seen as too similar. The authors used 112,120 chest ra-diographs from 30,805 patients for training, and for such a large dataset it is less likely that a diffusion model can memorize a large proportion of the images. Kazerouni et al. \cite{s-2} only mention privacy in a short paragraph in their survey.
% Why don’t gans investigate memorization?
% A possible explanation for this is that memorization has in general not been a problem for GANs, as the generator in a GAN never sees the training images directly (only indirectly through the discriminator). The architecture and loss function of GANs and diffusion models are completely different. While GANs use adversarial loss for training, diffusion models for example use mean squared error (between actual and estimated noise). These differences make it more likely for a diffusion model to memorize the training images [11].



% Here we compare a 2D GAN and a 2D diffusion model in terms of memorization, for synthetic brain tumor images, and demonstrate that diffusion models are much more prone to memorizing the training images. This can be very problematic in medical imaging where privacy is of uttermost importance. 
% In our previous work on ensembles of GANs [21,2], we trained segmentation networks using the synthetic images and used the obtained Dice scores for evaluation. When using synthetic images from diffusion models, it was observed that the Dice scores were as high as when training with real images, which made us suspicious. This work can be seen as a continuation of Carlini et al. [11] and Somepalli et al [33]., who investigated memorization for diffusion models but did not look into medical images, of Pinaya et al. \cite{mri-17} and Khader et al. \cite{mri-19} who used 3D diffusion models to synthesize brain volumes but did not look into memorization, of Dar et al. \cite{r-175} who looked into memorization for 3D diffusion models but did not compare with 3D GANs and of Packh ̈ auser et al. [24] who removed too similar synthetic images but did not report the significance of the problem






% \subsection{Generative models for MRI}
% \textbf{Effectiveness of generative models in addressing missing or corrupted contrasts in multi-contrast brain MRI:} Multiple studies have demonstrated the effectiveness of conditional generative models in synthesizing missing or corrupted contrasts in multi-contrast brain MRI. 

% \textbf{Limited evaluation of generated data's usefulness for downstream tasks:} Despite the advances in generating realistic synthetic MRI images, there is a need for more rigorous evaluation of the generated data's effectiveness for downstream tasks such as segmentation, classification, and disease diagnosis.

% \textbf{Limitations of existing studies:} Some studies have focused solely on qualitative evaluation of synthesis results without conducting usability studies. Additionally, many studies have been conducted on small datasets, limiting the generalizability of the findings.

% \textbf{Addressing the gap between real and synthetic data:} Existing studies suggest that there is still a gap between the realism and clinical relevance of synthetic data compared to real data. 

% \textbf{Image Quality Evaluation Metrics Not Specific to MRI:} The use of image quality evaluation metrics for synthetic MRI data is often based on metrics developed for natural images and may not adequately capture the unique characteristics of MRI modalities. For instance, FID (Fréchet Inception Distance) and IS (Inception Score) are widely used to evaluate the similarity between synthetic and real images, but they may not accurately reflect the subtle variations and noise patterns inherent in MRI data, as these metrics are  underpinned by a feature extractor pre-trained on the ImageNet dataset, which is more relevent for natural images.Additionally, these metrics may not fully capture the clinical relevance of synthetic data, as they do not directly address its impact on the performance of DL models for diagnostic or prognostic tasks.

% \textbf{Diversity is Important but Not Evaluated Properly:} The diversity of synthetic MRI data is crucial for ensuring that it encompasses the full range of anatomical and pathological variations encountered in clinical practice. However, many current methods for generating synthetic data focus on reproducing specific image characteristics rather than generating a truly diverse set of instances. This can lead to limitations in the generalizability of DL models trained on such data. A more comprehensive evaluation of synthetic MRI data should include measures of diversity, such as the range of anatomical features, pathological patterns, and image acquisition parameters.

% \textbf{Predominance of Intra-modality Translation for Brain MRI:} While there has been significant progress in developing synthetic MRI data for intra-modality translation, particularly between T1w, T2W, PD, and FLAIR sequences for brain imaging, the application of synthetic data to other modalities and organs remains limited. This is particularly concerning for cardiac MRI and breast MRI, where the lack of large, publicly available datasets poses a significant challenge for training DL models. Expanding the scope of synthetic data generation to incorporate these modalities and organs is crucial for advancing the application of DL in these areas of medical imaging.



The survey of the different papers across different data types and modalities reveal interesting insights that we categorize into goal of synthesis, generation methods, and evaluation methods.


\subsection{Goal of Synthesis}

\textbf{Diversity of clinically valid synthesis applications}:
Conditional generative models have demonstrated impressive capabilities in synthesizing missing or corrupted modalities across a diverse range of applications. As depicted in Fig.\ref{fig:synthesis-applications}, these applications vary depending on the data types involved. For example, in signals and images, both intra and inter modal translation between different modalities are common for various clinically valid reasons, such as synthesizing missing or corrupted MRI contrast when acquiring such images is not feasible or low-to-high density breast synthesis in mammograms or view conversion in Ultrasounds.  In the context of EHR, the synthesis and the choice of generative model depends on the specific format and requirements of the EHR data. For instance, the capability to manage high dimensionality is pivotal when handling longitudinal and aggregated EHR data, but its significance diminishes in the context of time-dependent and snapshot formats. Conversely, the preservation of temporal dependencies among clinical features remains crucial for both longitudinal and time-dependent formats. In medical text generation, the generated data serve multiple purposes beyond augmenting training data. They can be also used for NLP enhancement, such as entity extraction and question-answering systems, as well as text replacement for privacy reasons. 
 
% \textbf{Diversity of clinically valid Synthesis Applications-Related to  \ref{Synthesis Applications}}:  Multiple studies have demonstrated the effectiveness of conditional generative models in synthesizing missing or corrupted contrasts in multi-contrast brain MRI. While there has been significant progress in developing synthetic MRI data for intra-modality translation, particularly between T1w, T2W, PD, and FLAIR sequences for brain imaging, the application of synthetic data to other modalities and organs remains limited. This is particularly concerning for cardiac MRI and breast MRI, where the lack of large, publicly available datasets poses a significant challenge for training DL models. Expanding the scope of synthetic data generation to incorporate these modalities and organs is crucial for advancing the application of DL in these areas of medical imaging.
% In Mammograghy, this is evident, wehre multiple applications like low  to high density breast synthesis, view conversion, oppsosite breast synthesis,DFM to FFDM...Also evident in ultrasound, where view conversion and b-mode to Elastography US.
% Although the applications here are of huge clinical validity, it is rareley the case that they are properly evaluated clinically.

\textbf{Limited utilization of synthetic data beyond augmentation:} Despite its potential, synthetic data is underutilized beyond augmentation. This valuable resource, capable of generating diverse datasets varying in quality and anatomy, could serve as a comprehensive validation and testing set during model development. It has the potential to uncover algorithm limitations early on, particularly for challenging cases that may not be accessible due to data sharing policies or rarity, facilitating smoother translation of algorithms into clinical practice.  
[xray-3, xray-4, xray-6, xray-20, xray-21, oct-5, oct-15, oct-18, oct-21][ct-ot-15, ct-ot-33]










% \textbf{Limited utilization of synthetic data beyond augmentation:} Despite its potential, synthetic data is underutilized beyond augmentation. This data, with its ability to generate large-scale variable datasets varying in quality, noise, artifacts, anatomy, and appearance, offers an invaluable resource for rigorously assessing model performance and generalization during development. By serving as an extensive validation set, synthetic data can uncover algorithm limitations early in development, particularly for challenging cases that may be inaccessible due to data sharing policies or case rarity.Moreover, most medical analysis models and downstream models are shown to fail on out-of-distribution data that differ from those used for training, such as those acquired from different scanner vendors or acquisition sites. Synthetic data is promising for reducing this performance gap. 


% [xray-3, xray-4, xray-6, xray-20, xray-21, oct-5, oct-15, oct-18, oct-21][ct-ot-15, ct-ot-33]



\textbf{Most generative approaches are designed to handle the lack of training data but thorough analysis of how this is achieved is missing:} While numerous methodologies have been proposed to address the scarcity of training data, the specific elements of the generated data that contribute to improved outcomes remain largely unexplored. This is particularly true when the use of synthetic data alone does not yield any enhancement in performance [ct-ot-21, ct-lung-2, ct-lung-6, ct-lung-7, ct-lung-8, ct-lung-10, t-lung-16, ct-lung-21]. Only a handful of studies have indicated that the type of synthetic data incorporated into the training process can significantly impact results [ct-ot-23, xray-12]. For instance, incorporating challenging cases such as dense mammograms, severe examples of lung nodules in xray images or overlapping benign and malignant nodules in breast ultrasound, or underrepresented groups, has been shown to enhance performance. This underscores the potential benefits of active learning strategies, either during the data generation process or in selecting synthetic samples to be included in the training set.



\subsection{Generation}

 % \textbf{Choice of model depends on format and requirements of data}: The choice of generative model depends on the format of data at hand, especially in the case of EHR. For example, While the capability to manage high dimensionality is pivotal and frequently encountered in handling longitudinal and aggregated EHR data, its significance diminishes in the context of Time-dependent and Snapshot formats. In contrast, the preservation of temporal dependencies among clinical features remains crucial for both Longitudinal and Time-dependent formats.%EHR covered 


% \textbf{Diversity of clinically valid Synthesis Applications-Related to  \ref{Synthesis Applications}}:  Multiple studies have demonstrated the effectiveness of conditional generative models in synthesizing missing or corrupted contrasts in multi-contrast brain MRI. While there has been significant progress in developing synthetic MRI data for intra-modality translation, particularly between T1w, T2W, PD, and FLAIR sequences for brain imaging, the application of synthetic data to other modalities and organs remains limited. This is particularly concerning for cardiac MRI and breast MRI, where the lack of large, publicly available datasets poses a significant challenge for training DL models. Expanding the scope of synthetic data generation to incorporate these modalities and organs is crucial for advancing the application of DL in these areas of medical imaging.
% In Mammograghy, this is evident, wehre multiple applications like low  to high density breast synthesis, view conversion, oppsosite breast synthesis,DFM to FFDM...Also evident in ultrasound, where view conversion and b-mode to Elastography US.
% Although the applications here are of huge clinical validity, it is rareley the case that they are properly evaluated clinically.


\textbf{The leap of textual conditioning opens future directions:}
Recent advancements in text-conditional generative models offer an innovative approach to integrating descriptive data into synthetic medical data generation. This can involve structured text input specifying medical conditions and demographic data or utilizing medical reports as a source of clinically relevant guidance for the model.

\textbf{Conditional Models- Limited leverage of clinical knowledge, patient context, and text:}
A significant gap exists in the utilization of prior clinical knowledge, the availability of complimentary information accompanying the acquisition, as well as pathological processes,  biomarkers and radiology reports to inform the generation process. Most models fail to take advantage of these valuable resources, leading to potentially sub-optimal results. Similarly, conditioning based on subject characteristics patient and demographics is rarely utilized, except in isolated instances. This highlights the need to focus on more personalized synthesis tailored to specific subject characteristics and patient demographics, prioritizing fairness and inclusivity in medical data generation. Strong evidence suggests that conditional models leveraging such textual information, clinical knowledge, or other images/data inputs consistently produce higher quality and more realistic data compared to their non-conditional counterparts.



% \textbf{Conditional Models- Limited Leverage of Clinical Knowledge, Patient Context, and Text:}
% A significant gap exists in the utilization of prior clinical knowledge, complementary information like biomarkers and radiology reports, and patient demographics like age, sex, and ethnicity during the generation process. Most models fail to take advantage of these valuable resources, leading to potentially sub-optimal results. Recent advancements in text-conditional generative models offer an innovative approach to integrating this descriptive data into synthetic medical data generation. This can involve structured text input specifying medical conditions and demographic data or utilizing medical reports as a source of clinically relevant guidance for the model. In the medical text generation, the conditioning is applied to patients with certain diseases, conditions, or particular characteristics. However, their widespread adoption on generators for other data types remains limited. Similarly, conditioning based on subject characteristics and demographics is rarely utilized, except in isolated instances mentioned in the results and tables. This highlights the need to focus on more personalized synthesis tailored to specific subject characteristics and patient demographics, prioritizing fairness and inclusivity in medical data generation. Strong evidence suggests that conditional models leveraging such textual information, clinical knowledge, or other images consistently produce higher quality and more realistic data compared to their non-conditional counterparts.


% \textbf{The leap of Textual Conditioning opens future directions:}
% Recent advancements in text-conditional generative models offer an innovative approach to integrating descriptive data into synthetic medical data generation. This can involve structured text input specifying medical conditions and demographic data or utilizing medical reports as a source of clinically relevant guidance for the model.

% \textbf{Clinical prior knowledge rarely utilized to guide the generation process:} Most models do not take any advantage of prior clinical knowledge, the availability of complimentary information accompanying the acquisition, as well as pathological processes,  biomarkers and radiology reports to inform the generation process [ct-ot-7, ct-ot-10, ct-ot-14, ct-lung-15, oct-3, oct-4]. Rare models that present such solutions, might go for a  text-conditional generation approaches, and would typically produce synthetic images of better quality and diversity, with additional levels of control [ct-ot-8, ct-ot-10, ct-ot-12, ct-ot-17, ct-ot-19, ct-ot-20, ct-ot-21, ct-lung-1, ct-lung-3, ct-lung-13]. 

% \textbf{Insufficient Conditioning Based on Covariates:} A notable gap exists in the availability of conditional models that tailor generated data to specific subject characteristics and patient demographics, including factors such as age, sex, and BMI. Only in dermatology, \cite{derm-10}, and in mammography, \cite{mamm-4}, are there instances of models allowing for such conditioning. However, in ultrasound, no existing paper addresses this aspect, highlighting a need to consider fairness in medical practice.
% In EHR, only very few models \cite{ehr-25;ehr-59} allow conditional generation that considers static variables such as patient demographics, effectively addressing the needs of underrepresented subpopulations. However, Multiple models facilitate conditional generation tailored to specific medical conditions \cite{ehr-15} , with some focusing on the generation of uncommon diseases MTGAN and HALO \cite{ehr-22;ehr-38} .  %EHR covered


% % conditioning based on text can bee seen as a tool that allow for the previoous two: clinical prioir knowledge and conditioning on covariates.
% \textbf{Conditioning based on text:}Recent models have introduced an innovative approach by conditioning on clinical text, allowing the integration of descriptive data into synthetic medical data generation. This can involve 1) structured text input specifying medical conditions, and demographic data... or 2) medical reports that provide clinically relevant guidance to the model.  


% \textbf{Strong indication that conditional models generate higher quality and more realistic data}

\textbf{Limited tailoring of generative approaches to the specifics of medical data:} Most synthetic methods proposed for medical image generation still largely rely on loss functions and architectures initially designed for natural images, without considering the intricate aspects of medical image acquisition, physics and well defined statistics that can guide the generative process. Moreover, a significant number of models are designed to generate small patches (especially 3D) and lead to the generation of artificial features that can lead to large errors in anomaly detection and other tasks.  Computational limitations also restrict recent transformer-based approaches to slice-based training and diffusion models to low-resolution image generation.
In contrast, EHR generative models draw from established deep learning architectures like CTGANs but address unique challenges such as synthesizing mixed-type data with  static (e.g., demographics data) and sequential features (e.g., vital sign time-series), numerical features (e.g., blood pressure), and categorical features with many categories (e.g., medical codes). These models also prioritize modeling missing data patterns for informative analyses. Similarly, generative models for physiological signals leverage techniques for time-series data, some customizing to signal specifics like morphology or inter-lead relationships.
Regarding medical text generation, the application of pre-trained models and large language models has recently become prominent in the field. These models are based on general language models such as BERT and GPT and then adapted for medical applications through training or fine-tuning with specialized datasets, such as PubMed abstracts or clinical notes from the MIMIC database. However, this approach has limitations in that these advanced medical text generators may not fully grasp the underlying principles or logic of medical knowledge. 


% [ct-ot-7, ct-ot-14, ct-ot-20, ct-lung-13][ct-ot-11, ct-ot-16, ct-ot-28, ct-lung-11][ct-ot-11, ct-ot-12, ct-lung-21]
% \textbf{Design of generative approaches properly tailored to EHR:}
% While generative models for EHR may draw inspiration from components of common deep learning architectures and may be inspired by famous models for tabular data generation, such as Conditional Tabular GANs (CTGANs), the design goes beyond that to address specific challenges inherent to EHR data. This involves synthesizing mixed-type EHRs that comprise both static(e.g., demograghics data) and sequential data(e.g., vital sign time-series), numerical features (e.g., blood pressure), and categorical features with many categories (e.g., medical codes), ensuring that the models can effectively capture the inter dependencies among these diverse features. Moreover, multiple of these generative approaches recognize the significance of modeling missing data patterns,as they carry informative and relevant insights for analyses. These missingness patters reflect the reality of real-world healthcare data.  %EHR covered

% \textbf{Privacy is inherited in design in EHR}: In EHR, privacy preservation is claimed to be inherited in the design of the generative models. For instance, in the case of GANs, the model never directly observes the training images, accessing them only indirectly through the discriminator. This inherent privacy-by-design claim is substantiated through rigorous privacy evaluations.  While few exceptions explicitly integrate differential privacy into their architectural framework, some models take an additional step by implementing a relaxed variant of traditional differential privacy known as Renyi DP \cite{ehr-16}.%EHR covered- here, we can mention the work on privacy for images, like memoirzation.

\subsection{Evaluation}

% \textbf{Limitations of existing studies-MRI, to be merged with others:} Some studies have focused solely on qualitative evaluation of synthesis results without conducting usability studies for downstream tasks such as segmentation, classification, and disease diagnosis. 

\textbf{Limited benchmarking, comparative studies and the use of small private datasets}
The absence of comparative studies between different methods and the lack of a well-defined benchmark for comparison leaves a gap in understanding the relative strengths and weaknesses of various synthetic data generation approaches and therefore highlights the need for a more systematic approach. Moreover, the reliance on small, often private datasets for training and testing generative models raises concerns about the generalizability and usability of the generated data in clinical settings.  Most studies report both training and validation of the proposed synthesis approaches on significantly limited datasets - typically up to several hundreds of samples are used for training with a substantially smaller set for validation/testing. In addition, there is a severe lack of investigation of the effects of training data itself. 
% For instance, can accurate synthetic images be generated only by utilizing supervised translation approaches consisting of spatially registered samples versus using a significantly larger number of unpaired images.
 % [ct-lung-17]

% \textbf{Small datasets used for training and testing of generative models, which are often private:} Most studies report both training and validation of the proposed synthesis approaches on significantly limited datasets - typically up to several hundreds of images are used for training with a substantially smaller set for validation/testing. This raises serious doubts about the usability of generated data in clinical settings, as well as the ability of methods to produce diverse samples that are not just the copies of training data [ct-ot-31, ct-lung-5, ct-lung-7, ct-ot-20]. With the lack of proper evaluation methods that prove that synthetic data is clinically viable, small development datasets are a problem. In addition, there is a severe lack of investigation of the effects of training data itself [ct-lung-17]. For instance, can accurate synthetic images be generated only by utilizing supervised translation approaches consisting of spatially registered samples versus using a significantly larger number of unpaired images. Training and evaluation on private datasets is an additional problem, making the replication and comparison of proposed methods difficult.


% \textbf{Significant lack of proper clinical validation although crucial-The Missing Bridge to Practice:}  Although proposed for the use in clinical settings and downstream clinical analysis tasks, there is a significant lack of proper clinical validation reported. Studies that do perform clinical validation,  typically perform it on a small subset of clinical data, signifying a need for evaluation on large out-of-distribution internal and external validation datasets [ct-lung-5, ct-lung-12, ct-lung-13, ct-lung-19, ct-ot-22, ct-ot-28, ct-ot-30, ct-ot-33]. This lack and limitation of clinical evaluation hinders the translation of synthetic data from research into practice and prevents us from fully understanding its potential benefits and limitations. This is the case in EHR as well.%EHR covered


\textbf{Limited evaluation frameworks}: Most approaches focus on quantitative evaluation using fidelity metrics that are not designed for the specific kind of medical data. For example, in the case of medical images, the fidelity metrics employed are tailored for diverse data types such as natural images, overlooking the distinctive characteristics and statistical properties inherent to typical medical imaging modalities. Similarly, the evaluation metrics used for time-dependent EHR and physiological signals may overlook critical temporal features essential for an accurate evaluation. In medical text generation, there are no standards or well-accepted evaluation metrics to assess the fidelity of the generated data.  Sole reliance on such generic metrics, without incorporating additional measures of clinical validation, utility, and human visual perception studies can lead to misleading conclusions about the true quality and suitability of synthetic medical data. 

However, despite the crucial role of clinical validation in making sure that crucial anatomical details are maintained in the generated data, there is a notable lack in its proper implementation, hindering the translation of synthetic data into practical clinical settings. Studies that do perform clinical validation, typically perform it on a small subset of the generated data, signifying a need for evaluation on large internal and external validation datasets.

Moreover, human assessments are still limited and face significant design shortcomings. Typically, these studies involve a limited number of experts, often ranging from 1 to 3, which raises concerns about the statistical significance of the results. Furthermore, the design of these studies is often unclear, especially regarding the selection criteria of synthetic samples for evaluation. To enhance the effectiveness of these studies, they should be designed to gather reports from experts on indications that suggest certain samples are synthetic, providing the ability to correct for these artifacts in future approaches. In other instances, human visual assessment is reduced to a mere check of a few image samples for realism or a visual comparison of images from different methods, or merely inspecting visualizations such as PCA or t-SNE plots. 

A more comprehensive evaluation of synthetic data should include measures of diversity, ensuring that the synthetic data encompasses the full range of anatomical and pathological variations encountered in clinical practice. However, many current methods for generating synthetic data focus on reproducing specific image characteristics rather than generating a truly diverse set of instances. The lack of well-defined diversity metrics adds to the challenge, with researchers employing their own individual definitions.


\textbf{Limited evaluation of recent approaches based on diffusion and transformers:} Current research on diffusion models for data generation indicates they are more stable compared to GANs, with the ability to avoid mode collapse and vanishing gradients and add more control over the sampling process. However, a lot of diffusion models presented so far are yet to be properly tested and evaluated - utility studies are largely missing, as well as clinical validation or detailed qualitative and fidelity analysis of the generated data. Moreover, training is still performed on limited data that may lack adequate variability. 




% [ct-lung-12, ct-lung-18, ct-ot-3, ct-ot-6, ct-ot-16, ct-ot-19]. 


% \textbf{Diversity is Important but Not Evaluated Properly, nor well defined:} The diversity of synthetic data is crucial for ensuring that it encompasses the full range of anatomical and pathological variations encountered in clinical practice. However, many current methods for generating synthetic data focus on reproducing specific image characteristics rather than generating a truly diverse set of instances. This can lead to limitations in the generalizability of DL models trained on such data. A more comprehensive evaluation of synthetic  data should include measures of diversity, such as the range of anatomical features, pathological patterns, and image acquisition parameters.Moreover, researchers tend to have their own definitions of diversity each time in a paper.


% The current landscape of synthetic medical data generation faces significant challenges that extend beyond generic fidelity metrics. Privacy protection of generated medical images is inadequately evaluated, leaving uncertainties about data security. Challenges in human visual assessment studies, marked by limited expert involvement and unclear study designs, pose obstacles to reliable evaluations. Moreover, diversity in synthetic data, crucial for clinical practice, lacks a well-defined and properly evaluated framework.

\textbf{Privacy Disparities in Synthetic Medical Data:}
The assessment of privacy protection in generated medical data, encompassing images, EHR, and signals, faces notable disparities in standardized methodologies. Despite assertions of privacy capabilities and the potential for widespread data sharing, the absence of well-defined evaluation methods for medical images, signals, and text compared to EHR raises concerns. EHR privacy assessments commonly involve testing synthetic data for vulnerabilities against potential adversary attacks and demonstrating resilience against various threats. In contrast, privacy discussions in medical images primarily focus on the memorization of training data, leaving questions about identity disclosure unexplored. The extent to which generators and diffusion models memorize or replicate data, and their impact on tracing back learned distributions to original training data, remains unclear. While EHR benefits from established evaluation practices, addressing the significant gaps in privacy protection evaluation for other data types is crucial for ensuring the responsible deployment of synthetic data in medical contexts.

% The evaluation of privacy protection in generated medical images is currently marked by a significant lack of standardized methodologies. While many methods claim privacy capabilities and the potential for widespread data sharing, the absence of defined and rarely used evaluation methods raises concerns. In the context of medical images, the discussion about privacy converge to a discussion about memorization of the training data, without going into the details of identitiy disclosure. Yet,It is still not clear to what extent do generators and diffusion models memorize and/or replicate the data, nor how does that impact the ability to trace back the learned distributions to original training data. This lack of rigorous evaluation practices leaves the ethical and responsible application of synthetic images in sensitive medical contexts shrouded in uncertainty.
% In contrast, the evaluation of privacy protection in EHR is more standardized and extensive. EHR privacy evaluations commonly involve testing synthetic data for vulnerabilities against possible adversary attacks, showcasing resilience against various threats. However, this evaluation reveals a trade-off between privacy and utility, as some generative models, like TabDDPM, outperform GAN models across all metrics except privacy. Given the fact that privacy is rigorously evaluated in EHR, the claim that privacy is inherent in the design of the generative models is substantiated.  For instance, in the case of GANs, the model never directly observes the training images, accessing them only indirectly through the discriminator.While few exceptions explicitly integrate differential privacy into their architectural framework, some models take an additional step by implementing a relaxed variant of traditional differential privacy known as Renyi DP \cite{ehr-16}


%problem of assumed privay vs evaluated privacy





% \textbf{Privacy is inherited in design in EHR}: In EHR, privacy preservation is claimed to be inherited in the design of the generative models. For instance, in the case of GANs, the model never directly observes the training images, accessing them only indirectly through the discriminator. This inherent privacy-by-design claim is substantiated through rigorous privacy evaluations.  While few exceptions explicitly integrate differential privacy into their architectural framework, some models take an additional step by implementing a relaxed variant of traditional differential privacy known as Renyi DP \cite{ehr-16}.%EHR covered- here, we can mention the work on privacy for images, like memoirzation.



% \textbf{Significant lack of privacy protection evaluation of generated medical images: } Most methods suggest privacy protection capabilities of generated data and the potential for wide-scale data sharing; however, methods for evaluating the privacy are not defined and rarely used. It is still not clear to what extent do generators and diffusion models memorize and/or replicate the data, nor how does that impact the ability to trace back the learned distributions to original training data [ct-lung-8, ct-lung-9]. Without rigorous evaluation methodologies and standardized best practices in privacy protection, the ethical and responsible application of synthetic data in sensitive medical contexts remains shrouded in uncertainty.

% \textbf{Proper privacy protection evaluation of generated EHR}: In EHR, extensive Privacy evaluation is very common, and it typically includes testing the synthetic data for vulnerabilities against a possible adversary attack, with Many models showing resilience against various attacks. In some cases, the proposed generative model, such as TabDDPM, outperforms the GAN models across all evaluation metrics, except for privacy, which confirms the trade-off between privacy and utility. %EHR covered

% \textbf{Challenges in Human Visual Assessment Studies for Synthetic Data}: Despite their importance, particularly in the context of clinically and diagnostically relevant synthetic data, many human visual assessment studies face significant design shortcomings. Typically, these studies involve a limited number of experts, often ranging from 2 to 3, which raises concerns about the statistical significance of the results [ct-ot-4, ct-ot-5, ct-ot-31, ct-ot-32, ct-lung-1, ct-lung-3, ct-lung-14, ct-lung-17, ct-lung-19, oct-1, oct-4, oct-6, oct-10, oct-11]. Furthermore, the design of these studies is often unclear, especially in regard to the selection criteria of synthetic samples for evaluation [ct-ot-11, ct-lung-14, ct-lung-17, ct-lung-19]. In some instances, human visual assessment is reduced to a mere check of a few image samples for realism or a visual comparison of images from different methods,or merely inspecting visualizations such as PCA or t-SNE plots. Finally, To enhance the effectiveness of these studies, studies should be designed to gather the report from experts on indications that suggested certain samples are synthetic, providing the ability to correct for these artifacts in future approaches [ct-lung-19]. 


% \textbf{Flawed Metrics- A Misleading Lens}: Most approaches focus on quantitative evaluation using fidelity metrics that are not specifically designed for the specific kind of data. For example, in the case of medical images, the fidelity metrics used were originally designed for different types of images like natural images, not taking into account the characteristics and statistics of typical medical image modalities.  For instance, FID (Fréchet Inception Distance) and IS (Inception Score)  [oct-20, xray-15, xray-17, xray-18, xray-19, xray-22, ct-ot-1, ct-ot-3, ct-ot-6, ct-ot-9, ct-ot-13, ct-ot-14, ct-ot-19, ct-ot-27, ct-ot-29, ct-lung-16, ct-lung-18]  are widely used to evaluate the similarity between synthetic and real images, but they may not accurately reflect the subtle variations and noise patterns inherent in medical data, as these metrics are underpinned by a feature extractor pre-trained on the ImageNet dataset, which is more relevant for natural images. Similarly, the evaluation metrics used for time-dependent EHR are not speific to time-dependet data, and thus may miss an important aspect of the evaluation. Sole reliance on such generic metrics, without incorporating additional measures of clinical validation, utility, and  human visual perception studies can lead to misleading conclusions about the true quality and suitability of synthetic medical data [ct-lung-19].


% \textbf{Lack of comparative studies between different methods or a well-defined benchmark for comparison} [ct-lung-2, ct-lung-4, ct-lung-9, ct-lung-10, ct-lung-18, ct-ot-2, ct-ot-3, ct-ot-5, ct-ot-7, ct-ot-11, ct-ot-22, ct-ot-23, ct-ot-28, ct-ot-31, xray-5, xray-8, xray-9, xray-11-21, xray-23-26, oct-1, oct-4-6, oct-10, oct-13, oct-19-21, oct-23, oct-25  ] Navigating the landscape of synthetic data generation methods becomes challenging in the absence of well-defined benchmarks and comprehensive comparative studies. The lack of standardized evaluation frameworks and readily available benchmarks makes it difficult to assess and compare the performance of different approaches. This hinders the development and optimization of effective synthetic data generation methods tailored to specific healthcare needs. Comprehensive comparative studies employing established benchmarks would not only accelerate progress in the field but also provide valuable insights into the strengths and weaknesses of various techniques, guiding researchers towards the optimal tools for specific clinical applications.




==> ehr-new.tex <==

\subsection{EHR}
\label{sec:ehr}


EHRs are inherently heterogeneous, encompassing various types of data, including demographic data, ICD codes, and time-series vital signs, among others. They typically contain both static (e.g.: demographics) and sequential numerical features (e.g., blood pressure), as well as categorical features with many categories (e.g., medical codes). Given this complexity and heterogeneity, researchers and practitioners often differentiate four formats of EHR when developing generative models and generating synthetic data. These formats include longitudinal, time-dependent, aggregated, and snapshot, each with its own challenges and complexities, from modeling temporal dependencies and inter-dependencies between features to generating high-dimensional data and mixed-type features. Fig.\ref{fig:ehr-format} demonstrates different EHR data formats.

In this paper, we categorize the surveyed generative models according to these different EHR formats. We ensure to examine a multifaceted set of properties, each addressing a distinct aspect of the need for realistic heterogeneous EHR. These properties include preservation of temporal correlations and dependencies, ability for conditional generation, generation of uncommon diseases or underrepresented subpopulations, capability of handling high-dimensional formats, modeling missing patterns, and joint generation of static and temporal features. This comprehensive evaluation allows for a thorough assessment of the current state of synthetic data generation in the realm of EHR.

We start with an overview of early work in EHR synthesis (before the scope of this paper) and move to the different formats (Longitudinal, Time dependent, Aggregated, and Snapshot). A summary of the models is presented in Table.\ref{tab:ehr}, indicating the technology used for generation, type of features and different properties that the generative models are capable of, as well as the evaluation framework. 

% \begin{enumerate}
%     \item 	\textbf{Preservation of Temporal Correlations and Dependencies-(Temporal):} This property assesses whether the model can maintain the inherent time-based relationships present in the original EHR data, which is crucial for ensuring that temporal patterns, such as disease progression, are realistically replicated in the synthetic dataset.
%     \item 	\textbf{Ability for Conditional Generation-(Conditional):} Models are evaluated on their ability to generate data based on specific conditions or parameters. This capability allows for the creation of targeted datasets, such as those representing patient demographics or disease states.
%     \item 	\textbf{Generation of Uncommon Diseases or Underrepresented Subpopulations-(Rare):} A critical aspect of model evaluation is the ability to generate data for rare conditions or demographic groups that are typically underrepresented in datasets. This enhances the diversity and inclusiveness of the synthetic data.
%     \item 	\textbf{Capability of Generating High-Dimensional Formats-(High-dimensional):} High-dimensional data generation is essential for capturing the complexity of real-world EHRs, which often contain a vast number of variables. Models must be able to handle and accurately replicate these dimensions.
%     \item 	\textbf{Modeling Missing Patterns(Missingness): }The ability to model missing data patterns is important for producing synthetic datasets that reflect the reality of healthcare data, where missingness can be informative and relevant to analyses and play a key role in downstream predictive tasks \cite{che_Recurrent_2018}.
%     \item 	\textbf{Joint Generation of Static and Temporal Features(Joint):} Quality synthetic EHR data should encompass both static features (such as patient demographics) and temporal features (such as longitudinal clinical measurements), requiring models to jointly generate these feature types.
%     \item 	\textbf{Preserving Privacy (Privacy):} Given the sensitive nature of healthcare data, models must be evaluated on their ability to protect patient privacy, ensuring that the synthetic data cannot be used to identify individuals from the original dataset.
% \end{enumerate}

%%\label{}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{ehr-format.jpg}
    \caption{Different formats that EHR data exist in literature. \textbf{A. Longitudinal:}The most comprehensive yet least accessible due to privacy concerns, longitudinal EHRs track multiple attributes over the span of a patient’s life. A patient record $R_n$ consists of a sequence of visits of a patient to the healthcare provider $R_n = V_1, V_2, \ldots, V_T$, where each visit consists of a varying number of different data types (medical codes, lab results, diagnoses, clinical notes). In majority of cases, Each visit $V_t$ is a $K$-dimensional binary vector, where $V_T[k] = 1$ if the $k$-th code for patient $n$ was observed at visit $t$ and $0$ otherwise. $K$ denotes the cardinality of the set of possible codes.An Electronic Health Record (EHR) consists of a set of patient records $D = \{R_1, \ldots, R_n, \ldots, R_N\}$, where $N$ denotes the number of patients in the set. In this form, the temporal correlations between the visits should be maintained. \textbf{B. Time-dependent EHR:} This format captures regular, time-specific Data from monitoring devices, recorded at regular time intervals, focusing on physiological measurements such as Heart rate, respiratory rate,SpO2. \textbf{C. Aggregate:} This format flattens the diagnosis, medications, and procedure codes in the longitudinal data of a patient into aggregated data points represented in a single row with binary or count aggregations. The temporal and sequential aspect of the data is lost with this kind of processing, offering a cumulative overview instead \textbf{D. Snapshot or Cross-subsectional:} This is the most common format for public medical data, presenting a single static snapshot of a patient’s EHR focusing on selected attributes. }
    \label{fig:ehr-format}
\end{figure*}

% \begin{enumerate}
%     \item \textbf{Longitudinal:}The most comprehensive yet least accessible due to privacy concerns, longitudinal EHRs track multiple attributes over the span of a patient’s life. A patient record $R_n$ consists of a Visit sequence of visits of a patient to the healthcare provider $R_n = V_1, V_2, \ldots, V_T$, where each visit consists of a varying number of different data types (medical codes, lab results, diagnoses, clinical notes). In majority of cases, Each visit $V_t$ is a $K$-dimensional binary vector, where $V_T[k] = 1$ if the $k$-th code for patient $n$ was observed at visit $t$ and $0$ otherwise. $K$ denotes the cardinality of the set of possible codes.An Electronic Health Record (EHR) consists of a set of patient records $D = \{R_1, \ldots, R_n, \ldots, R_N\}$, where $N$ denotes the number of patients in the set. In this form, the temporal correlations between the visits should be maintained.
%     \item \textbf{Time-dependent EHR:} This format captures regular, time-specific Data from monitoring devices, recorded at regular time intervals, focusing on physiological measurements such as Heart rate, respiratory rate,SpO2. This format is complementary to longitudinal EHRs but more focused on continuous monitoring rather than episodic visits.
%     \item \textbf{Aggregate:} This format flattens the longitudinal data of a patient into aggregated data points represented in a single row, representing events with binary or count aggregations. The temporal and sequential aspect of the data is lost with this kind of processing, offering a cumulative overview instead. 
%     \item \textbf{Snapshot or Cross-subsectional:} This is the most common format for public medical data, presenting a single static snapshot of a patient’s EHR focusing on selected attributes. This format lacks historical context and provides a narrower overview than the Aggregated data.
% \end{enumerate}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!]
\centering
\tiny
\begin{tabular}{cccccc|cccccc|ccccccc|c}
\hline
\multirow{3}{*}{\textbf{Synthesis}} & \multirow{3}{*}{\textbf{Type}} & \multirow{3}{*}{\textbf{Features}} & \multirow{3}{*}{\textbf{Technology}} & \multirow{3}{*}{\textbf{Paper}} & \multirow{3}{*}{\textbf{DT}} & \multicolumn{6}{c|}{\textbf{Features}} & \multicolumn{7}{c|}{Evaluation} & \multirow{3}{*}{\textbf{Code}} \\ \cline{7-19}
 &  &  &  &  &  & \multirow{2}{*}{T} & \multirow{2}{*}{C} & \multirow{2}{*}{R} & \multirow{2}{*}{H} & \multirow{2}{*}{M} & \multirow{2}{*}{J} & \multicolumn{2}{c}{U} & \multirow{2}{*}{F} & \multirow{2}{*}{D} & \multirow{2}{*}{Q} & \multirow{2}{*}{C} & \multirow{2}{*}{P} &  \\ \cline{13-14}
 &  &  &  &  &  &  &  &  &  &  &  & Train & Test &  &  &  &  &  &  \\ \hline
\multirow{8}{*}{Longitudonal} & \multirow{3}{*}{GAN} & Dis & Two stage approach & SynTeg   \cite{s-36} & \textbf{Pred} & \checkmark (V) &  &  & \checkmark &  &  & S & R & \checkmark &  & \checkmark &  & \checkmark(inh) & \textbf{} \\
 &  & \multirow{2}{*}{Dis} & \multirow{2}{*}{WGAN-GP training- GRU gen} & \multirow{2}{*}{MTGAN \cite{ehr-22}} & \multirow{2}{*}{\textbf{Pred}} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c}{\multirow{2}{*}{*}} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  & \multicolumn{2}{c}{} &  &  &  &  &  &  \\
 & VAE & Dis & EHR VAE & EVA   \cite{ehr-15} & \textbf{Pred} & \checkmark & \checkmark & - & \checkmark &  &  & S,A & R & \checkmark & \checkmark & \checkmark &  & \checkmark(inh) &  \\
 & DM & Dis & DDPM based & MedDiffusion \cite{ehr-57} & \textbf{Pred} & \checkmark &  &  & \checkmark &  &  & \checkmark &  &  &  &  &  &  & \textbf{} \\
 & \multirow{3}{*}{LM} & Dis & Prompt based LM & PromptEHR   \cite{ehr-69} & \textbf{Pred} & \checkmark & \checkmark &  & \checkmark &  & \checkmark & S,A & R & \checkmark(Perp) &  &  &  & \checkmark(inh) & \checkmark \\
 &  & \multirow{2}{*}{Mix} & \multirow{2}{*}{hierarchical autoregressive LM} & \multirow{2}{*}{HALO \cite{ehr-38}} & \multirow{2}{*}{\textbf{Pred}} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{S,A} & \multirow{2}{*}{R} & \multirow{2}{*}{\checkmark(Perp)} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark(inh)} & \multirow{2}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{16}{*}{Timeseries} & \multirow{3}{*}{GAN} & \multirow{16}{*}{Mix} & \multirow{3}{*}{WGAN} & \multirow{3}{*}{HealthGAN \cite{ehr-13}} & \multirow{3}{*}{Class,Pred} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{S,R} & \multirow{3}{*}{S,R} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{2}{*}{\checkmark(inh)} & \multirow{3}{*}{} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & VAE &  & \begin{tabular}[c]{@{}c@{}}Dynamical VAE-architecture\\ with additional static component\end{tabular} & HealthGen   \cite{ehr-25} & Class & \checkmark & \checkmark & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & S & R & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \checkmark(inh) & \checkmark \\
 & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Hybrid :\\ VAE\\ +\\ GAN\end{tabular}} &  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}sequential enc-dec networks\\  followed by WGAN-GP\end{tabular}} & \multirow{2}{*}{EHR-safe \cite{s-18}} & \multirow{2}{*}{Class} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{\checkmark}} & \multirow{2}{*}{\textbf{\checkmark}} & \multirow{2}{*}{S} & \multirow{2}{*}{R} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{*}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\checkmark(inh)} & \multirow{2}{*}{} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  & \begin{tabular}[c]{@{}c@{}}LSTM based recurrent \\ AE and WGAN-GP\end{tabular} & LongGAN \cite{ehr-21} & Pred & \checkmark & \checkmark & \textbf{} & \textbf{} & \textbf{} & \textbf{} & S & R & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \checkmark(inh) &  \\
 &  &  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}dual LSTM based VAE, \\ bilateral LSTM gen\\ and LSTM dis\end{tabular}} & \multirow{3}{*}{EHR-M-GAN \cite{s-10}} & \multirow{3}{*}{Class} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\textbf{-}} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{S,A} & \multirow{3}{*}{R} & \multirow{3}{*}{\checkmark(time)} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{\textbf{}} & \multirow{3}{*}{\checkmark(DP)} & \multirow{3}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  & \begin{tabular}[c]{@{}c@{}}Combined Time-GAN\\  and ADS-GAN\end{tabular} & Time-ADS-GAN \cite{TIME-ADS-GAN} & Pred & \checkmark &  &  &  &  & \textbf{\checkmark} & S & R & \checkmark & \checkmark & \textbf{*} & \textbf{} & \textbf{\checkmark(ϵ)} &  \\
 & \multirow{5}{*}{DM} &  & \begin{tabular}[c]{@{}c@{}}DDPM, with postporcessing \\ of output\end{tabular} & EHR-DPM \cite{s-34} & RL & \checkmark & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{\checkmark} & S & R & \checkmark & \textbf{\checkmark} & \textbf{} & \textbf{} & \checkmark(inh) &  \\
 &  &  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}mixed sequence DDPM \\ with BRNN denoiser\end{tabular}} & \multirow{4}{*}{TIMEDIFF \cite{ehr-58}} & \multirow{4}{*}{Pred} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{\checkmark}} & \multirow{4}{*}{\textbf{\checkmark}} & \multirow{4}{*}{S,A} & \multirow{4}{*}{R} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{*}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\checkmark(inh)} & \multirow{4}{*}{*} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Aggregate,\\ Signals, \\ and Snapshot\end{tabular}} & \multirow{7}{*}{GAN} & \multirow{7}{*}{Dis} & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}convolutional AE \\ and convolutional GAN\end{tabular}} & \multirow{7}{*}{RDP-CGAN \cite{ehr-16}} & \multirow{7}{*}{None} & \multirow{7}{*}{\checkmark} & \multirow{7}{*}{\checkmark} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{\checkmark} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{} & \multirow{7}{*}{} & \multirow{7}{*}{\checkmark} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{\textbf{}} & \multirow{7}{*}{\textbf{\checkmark(Renyi DP)}} & \multirow{7}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{Aggregate} & GAN & Mix & \begin{tabular}[c]{@{}c@{}}based on \\ EMR-WGAN\end{tabular} & HGAN   \cite{s-41} & None & \textbf{} & \checkmark & \textbf{-} & \checkmark & \textbf{} & \textbf{} &  &  & \checkmark & \textbf{} & \textbf{} & \textbf{} & \checkmark(inh) & \textbf{} \\
 & \multirow{3}{*}{DM} & \multirow{2}{*}{Mix} & \multirow{2}{*}{AE followed by SDE} & \multirow{2}{*}{ScoEHR    \cite{s-24}} & \multirow{2}{*}{Class} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{SRA}}} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{(inh)} & \multirow{2}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  & \multicolumn{2}{c}{} &  &  &  &  &  &  \\
 &  & Dis & SDE & EHRDIFF \cite{s-11} & Class & \textbf{} & \textbf{} & \textbf{} & \checkmark & \textbf{} & \textbf{} &  &  & \checkmark & \textbf{\checkmark} & \textbf{} & \textbf{} & \checkmark(inh) & \checkmark \\
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Aggregate, \\ and Snapshot\end{tabular}} & \multirow{6}{*}{DM} & \multirow{2}{*}{D*,C} & \multirow{2}{*}{DDPM,modified U-net} & \multirow{2}{*}{MedDiff \cite{s-15}} & \multirow{2}{*}{Class} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{S} & \multirow{2}{*}{R} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  & \multirow{4}{*}{D*,M} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}mixed sequence DDPM,\\  with MLP Denoiser\end{tabular}} & \multirow{4}{*}{TabDDPM \cite{s-12}} & \multirow{4}{*}{Class} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{S,A} & \multirow{4}{*}{R} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\checkmark(inh)} & \multirow{4}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{14}{*}{Snapshot} & \multirow{14}{*}{GAN} & \multirow{14}{*}{Mix} & \begin{tabular}[c]{@{}c@{}}WGAN-GP  based, \\ preceeded by data\\  transofrmations\end{tabular} & HealthGAN \cite{ehr-59} & None & \textbf{} & \textbf{} & \textbf{} & \checkmark & \textbf{} & \textbf{} &  &  & \checkmark & \textbf{} & \textbf{*} & \textbf{} & \checkmark(inh) & \textbf{} \\
 &  &  & \multirow{4}{*}{WGAN-GP based} & \multirow{4}{*}{ADS-GAN \cite{ehr-12}} & \multirow{4}{*}{Pred} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{*}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{S} & \multirow{4}{*}{R} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{}} & \multirow{4}{*}{\textbf{\checkmark (ϵ)}} & \multirow{4}{*}{\textbf{}} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  & MLP  gen and disc & Pgan \cite{ehr-26} & Class,Reg & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & S & R & \textbf{} & \textbf{} & \textbf{*} & \textbf{} & \checkmark(inh) & \textbf{} \\
 &  &  & \multirow{8}{*}{CTGAN} & \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}CTGAN \\ \cite{ehr-24,ehr-50,ehr-47,ehr-52}\end{tabular}} & \multirow{8}{*}{Class} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\checkmark} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{S,A} & \multirow{8}{*}{R} & \multirow{8}{*}{\checkmark} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\textbf{}} & \multirow{8}{*}{\checkmark} \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\caption{*  meaning: in T: Visit level- in U:pretrain on synthetic, then fine tune on real, ϵ-identifiability- The table lists the key properties evaluated for generative models of EHRs, including (T) preservation of temporal correlations and dependencies, (C) ability for conditional generation, (R) generation of uncommon diseases or underrepresented subpopulations, (H) capability of generating high-dimensional formats, (M) modeling missing patterns, (J)joint generation of static and temporal features. In the privacy column of the evaluation, the checkmark indicates the presence of privacy evaluation, while the text in paranthesis indicate the method that the model follow to preserve privacy. In majority of the cases, the privacy is inherent, meaning that it is assumed in the design of the model.}
\label{tab:ehr}
\end{table*}


\subsubsection{Early work on EHR }

Most GANs were designed for continuous data coming from the imaging domain. For this reason, Early works on GANs for EHRs (before the scope of this survey) were centered around producing structured, discrete tabular EHRs, including diagnosis and billing ICD codes. The initial GAN architecture that generated discrete EHR, medGAN, released in 2017, utilized an autoencoder to address the original GAN architecture’s inability to generate discrete features in combination with a mini-batch averaging to mitigate mode collapse \hl{[s-13]}. Following the success of medGAN in generating discrete data, medWGAN and medBGAN \hl{[s-16]} were introduced, replacing the standard GAN with a  Wasserstein GAN with gradient penalty (WGAN-GP) \hl{[32]} and boundary-seeking GANs (BGAN) \hl{[91]}, respectively. The authors notably contributed to enhancing the quality of the generated data, surpassing that of the original medGAN. In MC-medGAN, adaptations to medGAN were proposed to facilitate a superior representation of multi-categorical data \hl{[s-35]}. Other endeavors have concentrated on enhancing training stability, such as the approach proposed in EMR Wasserstein GAN (EMR-WGAN) \hl{[s-17]}. It omits the autoencoder in medGAN and enabled the generator to directly output synthetic data. The authors also implemented a filtering strategy to boost GANs training for low-prevalence clinical concepts. 

After that, the work proceeded, expanding the scope to cover not only discrete feature types but heterogeneous type (continuous and discrete) as well, and model temporal correlations as well.


\subsubsection{Generative Models- Longitudinal Format }

% \begin{table*}[ht]
% \centering
% \footnotesize
% \begin{tabular}{|C{2cm}|C{2cm}|C{2cm} C{2cm} C{2cm} C{2cm} C{2cm}|}
% \hline
% \textbf{Feature/Model} & \textbf{SynTeg} & \multicolumn{1}{C{2cm}|}{\textbf{EVA}} & \multicolumn{1}{C{2cm}|}{\textbf{MTGAN}} & \multicolumn{1}{C{2cm}|}{\textbf{HALO}} & \multicolumn{1}{C{2cm}|}{\textbf{MedDiffusion}} & \textbf{PromptEHR} \\ \hline
% \textbf{Type} & GAN & \multicolumn{1}{C{2cm}|}{VAE} & \multicolumn{1}{C{2cm}|}{GAN} & \multicolumn{1}{C{2cm}|}{LM} & \multicolumn{1}{C{2cm}|}{DM} & LM \\ \hline
% \textbf{Date} & Nov-20 & \multicolumn{1}{C{2cm}|}{Dec-20} & \multicolumn{1}{C{2cm}|}{Apr-22} & \multicolumn{1}{C{2cm}|}{Mar-23} & \multicolumn{1}{C{2cm}|}{Oct-23} & Oct-22 \\ \hline
% \textbf{Feature Types} & Dis & \multicolumn{1}{C{2cm}|}{Dis} & \multicolumn{1}{C{2cm}|}{Dis} & \multicolumn{1}{C{2cm}|}{Mix} & \multicolumn{1}{C{2cm}|}{Dis} & Dis \\ \hline
% \textbf{Datasets} & VUMC SD & \multicolumn{1}{C{2cm}|}{SHPAMF} & \multicolumn{1}{C{2cm}|}{MIMIC-III,IV} & \multicolumn{1}{C{2cm}|}{OPeHR,MIMIC-III} & \multicolumn{1}{C{2cm}|}{MIMIC+} & MIMIC-III \\ \hline
% \textbf{Downstream Task} & - & \multicolumn{5}{c|}{Pred} \\ \hline
% \textbf{Temporal} &\checkmark (Visit level) & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} &\checkmark \\ \hline
% \textbf{Conditional} & x & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} &\checkmark \\ \hline
% \textbf{Rare} & x & \multicolumn{1}{C{2cm}|}{-} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} & * \\ \hline
% \textbf{High dimension} &\checkmark & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark \checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} &\checkmark \\ \hline
% \textbf{Missingness} & x & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & x \\ \hline
% \textbf{Joint} & x & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} &\checkmark \\ \hline
% \textbf{Privacy} &\checkmark (inherited) & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \multicolumn{1}{C{2cm}|}{*} & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \multicolumn{1}{C{2cm}|}{*} &\checkmark (inherited) \\ \hline
% \end{tabular}
% \caption{\textbf{EHR Longitudonal format}- * not mentioned/evaluated; MIMIC+- MIMIC ,Amnesia,COPD,Kideny ; SHPAMF- Sutter Health Palo Alto Medical Foundation; Pred-Prediction;LM-Language Model}
% \label{tab:ehr-longitudonal}
% \end{table*}


\paragraph{EHR requirements}Table.\ref{tab:ehr} summarizes several models that generate synthetic longitudinal EHR data, emphasizing their ability to handle the \textit{high dimensionality} of medical datasets, mainly discrete features, such as those including ICD-9 codes. These models are adept at preserving \textit{temporal correlations across patient visits}, with  \cite{s-36}  additionally maintaining these correlations at the visit level. Despite their capabilities, none of the models explicitly address the patterns of missing data in their design. 

% .

\paragraph{Generation} Beside GANs, VAE, DM, and LM have been utilized to generate longitudonal \textbf{EHR}. The authors Of \cite{s-36} approached the problem using a two-stage strategy. The initial stage sequentially estimates temporal patterns and expected patient state from visits, incorporating a self-attention layer and using recurrent neural netwroks (RNN). The subsequent stage generates data, conditioned on the expected patient state, utilizing Wasserstein GAN \hl{[31]} and the previous EMR-WGAN work. The generator of the model in \cite{ehr-22} uses WGAN-GP  with a gated recurrent unit (GRU) generator to generate sequences and adopt the concept of a smooth conditional matrix from CTGANs \hl{[source]} to generate uncommon diseases, and the discriminator uses Wasserstein distance considering both data and temporal features. The authors also design a training strategy to optimize the model by sampling discrete diseases from visit-level probabilities and forming the patient-level visit sequences to stabilize the training process. 

The models in \cite{ehr-38} and \cite{ehr-69} stand out by following a language model approach, with \cite{ehr-38} using Hierarchical Autoregressive Language model, treating EHR data as natural language sequences, uniquely capable of synthesizing both discrete (medical codes) and continuous (average values of lab tests) data types, emulating the heterogeneous character of EHRs. It does this through granular discretization, capturing the full spectrum of static and temporal patient features. The model in \cite{ehr-69} offers the flexibility to modulate diversity using a variety of methods found in the natural language generation literature. This is in contrast to GANs and VAEs, which rely on the sampling of random noise vectors to inject diversity. Such an approach is not only uncontrollable but often compromises the quality of the generated content.


\paragraph{Conditioning} Several models incorporate conditional generation to enhance the utility and specificity of the generated data. The model in \cite{ehr-15} facilitates conditional generation tailored to specific medical conditions. \cite{ehr-22} is focused on the generation of uncommon diseases, which is particularly beneficial for downstream tasks involving these less frequent conditions. Finally, \cite{ehr-38} uses demographic and chronic disease phenotypes for conditional generation, which helps create balanced datasets for training downstream tasks on rare conditions.

\paragraph{Privacy and Evaluation} Models outlined in the table are designed with inherent privacy-preserving features within their architectural frameworks, and privacy evaluation is performed in most cases. While all models were evaluated for their utility in downstream tasks specifically for training downstream AI models or augmenting the training set, the diffusion model in \cite{ehr-57} lacked fidelity evaluation. Iconically, \cite{ehr-22} evaluate for the generated disease types, which is concerned with the presence and representation of all possible categories, usually diseases, and medical codes, in the synthetic data.\cite{s-36} refers to human experts to classify the synthetic data as looking real or fake. %TODO: Talk abou tperplexity


\subsubsection{Generative Models- Time-dependent Format }


% \begin{table*}[h]
% \centering
% \footnotesize

% \begin{tabular}{|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
% \hline
% \textbf{Feature/Model} & \multicolumn{1}{C{2cm}|}{\textbf{HealthGAN (WGAN) \cite{ehr-13}}} & \multicolumn{1}{C{2cm}|}{\textbf{EHR-M-GAN \cite{s-10}}} & \multicolumn{1}{C{2cm}|}{\textbf{LongGAN \cite{ehr-21}}} & \multicolumn{1}{C{2cm}|}{\textbf{HealthGen \cite{ehr-25}}} & \multicolumn{1}{C{2cm}|}{\textbf{EHR-safe \cite{s-18}}} & \multicolumn{1}{C{2cm}|}{\textbf{EHR-DPM \cite{s-34}}} & \textbf{TIMEDIFF \cite{ehr-58}} \\ \hline
% \textbf{Type} & \multicolumn{1}{C{2cm}|}{GAN} & \multicolumn{1}{C{2cm}|}{GAN} & \multicolumn{1}{C{2cm}|}{GAN} & \multicolumn{1}{C{2cm}|}{VAE} & \multicolumn{1}{C{2cm}|}{GAN} & \multicolumn{1}{C{2cm}|}{DM} & DM \\ \hline
%  \textbf{Technology} &\multicolumn{1}{C{2cm}|}{} & \multicolumn{1}{C{2cm}|}{dual VAE, bilateral LSTM generator} & \multicolumn{1}{C{2cm}|}{recurrent autoencoders and WGAN-GP} & \multicolumn{1}{C{2cm}|}{} & \multicolumn{1}{C{2cm}|}{sequential encoder-decoder networks and GANs} & \multicolumn{1}{C{2cm}|}{DPM} & DDPM, with BRNN \\ \hline
% \textbf{Date} & \multicolumn{1}{C{2cm}|}{Sep-20} & \multicolumn{1}{C{2cm}|}{Dec-21} & \multicolumn{1}{C{2cm}|}{Jan-22} & \multicolumn{1}{C{2cm}|}{Jul-22} & \multicolumn{1}{C{2cm}|}{Dec-22} & \multicolumn{1}{C{2cm}|}{Mar-23} & Oct-23 \\ \hline
% \textbf{Feature Types} & \multicolumn{7}{c|}{Mixed} \\ \hline
% \textbf{Datasets} & \multicolumn{1}{C{2cm}|}{MIMIC-III} & \multicolumn{1}{C{2cm}|}{MIMIC-III,HIRD,eICU} & \multicolumn{1}{C{2cm}|}{CHF} & \multicolumn{1}{C{2cm}|}{MIMIC-III} & \multicolumn{1}{C{2cm}|}{MIMIC-III,eICU} & \multicolumn{1}{C{2cm}|}{MIMIC-III, ART for HIV} & MIMIC-III,IV,HIRD,eICU \\ \hline
% \textbf{Downstream Task} & \multicolumn{1}{C{2cm}|}{Class and Pred} & \multicolumn{1}{C{2cm}|}{Class} & \multicolumn{1}{C{2cm}|}{Pred} & \multicolumn{1}{C{2cm}|}{Class} & \multicolumn{1}{C{2cm}|}{Class} & \multicolumn{1}{C{2cm}|}{Reinf} & - \\ \hline
% \textbf{Temporal} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \checkmark \\ \hline
% \textbf{Conditional} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & x \\ \hline
% \textbf{Rare} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{-} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & x \\ \hline
% \textbf{High dimension} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & x \\ \hline
% \textbf{Missingness} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{x} & \checkmark \\ \hline
% \textbf{Joint} & \multicolumn{1}{C{2cm}|}{} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{x} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark} & \checkmark \\ \hline
% \textbf{Privacy} & \multicolumn{1}{C{2cm}|}{\checkmark} & \multicolumn{1}{C{2cm}|}{\checkmark (DP)} & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \multicolumn{1}{C{2cm}|}{\checkmark (inherited)} & \checkmark (inherited) \\ \hline
% \end{tabular}
% \caption{\textbf{Time-dependent Format}- Class-Classification, Pred-Prediction,Reinf-Reinforcement Learning, CHF-Cerner Health Facts database, DP-Differential Privacy}
% \label{tab:ehr-time}
% \end{table*}

%technologies


\paragraph{EHR requirements}The capacity to preserve \textit{temporal dependencie}s and correlations among clinical features is a critical functionality for models generating synthetic time dependent EHR data. The challenge of \textit{high-dimensional} data generation is less pronounced in time-dependent than longitudinal format since the extensive data typically associated with medical codes is not utilized. The WGAN based model\cite{ehr-13} is the exception, with the ability to generate high-dimensional, time-dependent records featuring 714 attributes. Conversely, \cite{s-10}, in its initial design, limited the dimensionality of variables to less than 100, potentially constraining its capacity to represent the complexity of medical data fully. Models like the ones in\cite{s-18}, \cite{s-34},\cite{ehr-25}, and \cite{ehr-58} focus as well on accurately reflecting the heterogeneous nature of real-world EHR through a \textit{combination of static and temporal features}.  \cite{ehr-25,s-18,ehr-58} are all proficient in handling \textit{missingness patterns}, a critical aspect that \cite{ehr-21} opts to eliminate through data imputation, potentially losing valuable information inherent in the absence of data. Iconically, \cite{s-18} manages varying time-series sequence lengths.



\paragraph{Generation} \cite{ehr-13} adeptly transforms longitudinal patient data into a cross-subsectional format while maintaining these temporal dependencies, applying a WGAN. The idea of combining an autoencoder with a GAN is widely used, mainly to establish a shared latent space representation encompassing mixed types of EHRs features, including both continuous and discrete-valued data, prior to the generation process. For instance, both \cite{ehr-21} and \cite{s-18} employ autoencoder networks followed by a WGAN-GP. \cite{ehr-21} utilizes a LSTM based recurrent autoencoder, while  \cite{s-18} employs a sequential encoder-decoder network. Expanding upon this strategy, \cite{s-10} incorporates a dual LSTM-based VAE. It then employs bilaterally coupled LSTM GANs to ensure capturing temporal correlations within diverse EHR types.  \cite{TIME-ADS-GAN} combines research on time-dependent synthetic data (TimeGAN) and  privacy preserving static synthetic data (ADS-GAN  \cite{ehr-12}), where The TimeGAN also utilize the latent space of the autoencoder for better synthesis.

 \cite{s-34} and  \cite{ehr-58} are novel approaches that utilize diffusion models to generate mixed type data. While \cite{s-34} resorts to Gaussian diffusion for generating discrete sequences, treating them similarly to real-valued sequences but with further post-processing of the model output,  \cite{ehr-58} on the other hand simultaneously generates (without need for post-processing) time series discrete (using multinomial diffusion) and continuous (using Gaussian diffusion) data that preserve temporal dependencies because of the use of a BRNN instead of U-net in the backward diffusion step. 


\paragraph{Conditioning}\textit{Conditional generation} is a capability shared by several models, including \cite{ehr-13,s-10,ehr-21,ehr-25}.  \cite{s-10} utilizes condition-specific labels(outcomes: ICU mortality, hospital mortality, 30-day re-admission, hospital discharge…) to improve model performance, although its conditional generation capabilities are limited and not extendable to patient-specific EHRs based on detailed information such as patient demographics. In contrast, \cite{ehr-25} excels in this area by enabling conditional generation that considers static variables, effectively addressing the needs of \textit{underrepresented sub-populations} and contributing to fairness in downstream machine learning applications.


% Privacy is another pivotal concern in EHR data generation. Models like DP-CTGAN and PATE-CTGAN  \cite{ehr-30} prioritize this by generating continuous heart monitoring data with an eye on privacy. 

\paragraph{Evaluation and Privacy}\cite{s-10} explicitly incorporates differential privacy into its architecture. \cite{ehr-25} indirectly supports privacy by ensuring that synthetic data do not replicate the training data. All models other than \cite{s-10}, although lacking explicit theoretical privacy guarantees, shows empirical resilience against various adversary privacy attacks. While all models were evaluated for their utility, only \cite{s-34} conducted a diversity analysis to evaluate the coverage of all demographic features present in the real dataset as well as uniquely evaluating the utility of their model for the downstream task of reinforcement learning. 
However, a limitation in the evaluation of this form of time-dependent synthetic EHR arises from the scarcity of time-specific metrics. Instead, the authors opted to assess the temporal aspect of the data by evaluating the utility for temporal tasks.


\subsubsection{Generative Models- Aggregated Format }

% \begin{table*}[ht]
% \centering
% \footnotesize

% \begin{tabular}{|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
% \hline
% \textbf{Model} & \textbf{RDP-CGAN \cite{ehr-16}} & \textbf{HGAN \cite{s-41}} & \textbf{ScoEHR \cite{s-24}} & \textbf{MedDiff \cite{s-15}} & \textbf{EHRDIFF \cite{s-11}} & \textbf{TabDDPM \cite{s-12}} \\ \hline
% \textbf{Type} & \multicolumn{2}{C{4cm}|}{GAN} & \multicolumn{4}{c|}{DM} \\ \hline
% \textbf{Technology} & Conv AE and Conv GAN & Based on EMR-WGAN & & & Stochastic Differential Equations & DDPM \\ \hline
% \textbf{Year} & Dec-20 & Jun-21 & Jan-23 & Feb-23 & Mar-23 & Aug-23 \\ \hline
% \textbf{Datasets} & MIMIC-III & VUMC Synthetic Derivative & MIMIC, ED-EHR & MIMIC & MIMIC-III & MIMIC-III \\ \hline
% \textbf{Feature Type} & Dis & Mix & Mix & Dis & Dis & Discrete \\ \hline
% \textbf{Downstream Task} & & & Class & Class & Class & Class \\ \hline
% \textbf{Temporal} & \checkmark & x & x & x & x & x \\ \hline
% \textbf{Conditional} & \checkmark & \checkmark & x & \checkmark & x & x \\ \hline
% \textbf{Rare} & x & - & x & x & x & x \\ \hline
% \textbf{High Dimension} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
% \textbf{Missingness} & x & x & x & x & x & x \\ \hline
% \textbf{Joint} & x & x & x & x & x & x \\ \hline
% \textbf{Privacy} & \checkmark (Renyi DP) & \checkmark (Inherited) & \checkmark (Inherited) & * & \checkmark (Inherited) & Worst compared to other methods \\ \hline
% \end{tabular}
% \caption{\textbf{Aggregated} EHR- *not mentioned/evaluated; Conv:Convolutional}
% \label{tab:my-table}
% \end{table*}

\paragraph{EHR requirements:} In the context of aggregated format generation for electronic health record (EHR) data, all models demonstrate a range of capabilities, particularly in \textit{handling high-dimensional data}. Models such as HGAN \cite{s-41} and ScoEHR \cite{s-24} adept at managing the complex and multifaceted nature of EHR data that often involves mixed feature types (continuous and discrete). However, a significant limitation across all these models is their lack of consideration for \textit{missing data patterns}. Additionally, they do not integrate both static features, like patient demographics, and temporal features, such as medical readings over time, in their generation process. This gap limits their ability to fully replicate the nuanced and comprehensive nature of real-world EHR data. Beyond the primary focus on aggregated format EHR, several models have also shown effectiveness in other data formats.  RDP-CGAN \cite{ehr-16}, for example, have been effective with EEG and ECG data, demonstrating their ability to preserve temporal correlations and maintain the integrity of time-series patterns. Additionally, RDP-CGAN, MedDiff \cite{s-15}, and TabDDPM \cite{s-12} have proven effective in generating snapshot format data as well.


\paragraph{Generation:} Although most old work has been focusing on this format of data, more research has been conducted in this direction, utilizing recent diffusion models for this task. ScoEHR was the first to do so, followed by MedDiff, and EHRDIFF. ScoEHR \cite{s-24} compress the high-dimensional mixed features into a low-dimensional representation and perform SDE diffusion in the latent space, while EHRDIFF\cite{s-21} apply SDE directly to discrete values, treating them like continuous numbers. MedDIFF \cite{s-15}, on the other hand, use a DDPM without requiring a pre-trained encoder, utilizing a modified U-net using 1D convolutional layers to accompany the tabular type of data, while TabDDPM \cite{s-12} follow a mixed diffusion approach to generate realistic mixed-type tabular EHRs.  

% RDP-CGAN \cite{ehr-16} employs a convolutional AE and convolutional GAN, while the model in \cite{s-41} is based on EMR-WGAN.
\paragraph{Conditioning:} Concerning conditional generation, HGAN, RDP-CGAN, and MedDiff support this functionality, with HGAN allowing for conditioning on demographic features such as age and gender, while MedDiff facilitates class-based conditioning  by incorporating the idea of a classifier-guided sampling process. Despite these capabilities, these models do not specifically focus on generating data for uncommon diseases or underrepresented conditions, potentially overlooking important aspects of healthcare diversity.

\paragraph{Evaluation and Privacy:} Privacy remains a pivotal concern, with HGAN, ScoEHR, and EHRDIFF demonstrating a low risk of privacy attacks. However, there's room for improvement in their privacy mechanisms, such as the potential incorporation of differential privacy, rather than relying solely on inherited privacy traits. RDP-CGAN stands out by explicitly implementing Renyi DP, a relaxed variant of traditional differential privacy. Meanwhile, TabDDPM, despite its excellence in data quality, utility, and augmentation, faces challenges in privacy, underscoring the often present trade-off between privacy and utility in synthetic data generation. 


\subsubsection{Generative Models- Snapshot Format }

% \begin{table*}[]
% \centering
% \footnotesize
% \begin{tabular}{|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
% \hline
% \textbf{Model} & \textbf{HealthGAN \cite{ehr-59}} & \textbf{ADS-GAN \cite{ehr-12}} & \textbf{Pgan \cite{ehr-26}} & \textbf{CTGAN \cite{ehr-50}} & \textbf{CTGAN \cite{ehr-52}} \\ \hline
% \textbf{Type} & \multicolumn{5}{c|}{GAN} \\ \hline
% \textbf{Year} & Nov-20 & Aug-20 & Sep-22 & Feb-22 & Jun-23 \\ \hline
% \textbf{Feature Type} & Mixed & Mixed & Mixed & Mixed & Mixed \\ \hline
% \textbf{Datasets} & MIMIC-III & MAGGIC, UNOS & PIMA & Misc. & NY \\ \hline
% \textbf{Downstream Task} & & Pred & Class and Reg & Class & Pred \\ \hline
% \textbf{Temporal} & x & x & x & x & x \\ \hline
% \textbf{Conditional} & X & * & x & \checkmark & \checkmark \\ \hline
% \textbf{Rare} & X & x & x & x & x \\ \hline
% \textbf{High Dimension} & \checkmark & x & x & x & x \\ \hline
% \textbf{Missingness} & X & x & x & x & x \\ \hline
% \textbf{Joint} & x & x & x & x & x \\ \hline
% \textbf{Privacy} & \checkmark & \checkmark ($\epsilon$-identifiability)& \checkmark & not mentioned/evaluated & \checkmark \\ \hline
% \end{tabular}
% \caption{\textbf{Snapshot} EHR- PIMA- PIMA Indian diabetes dataset,NY-NY Hospital Inpatient Discharges in 2015,Pred-Prediction, Class-Classification, * opimized }
% \label{tab:ehr-snapshot}
% \end{table*}


\paragraph{EHR requirements:} As the snapshot format lack the time aspect, none of the models are designed to preserve temporal correlations within the datasets they handle. \textbf{HealthGAN} \cite{ehr-59} stands out as the only model capable of handling high-dimensional data (handling 324 features). Missing data patterns are not addressed by any of the models, nor the joint static and temporal features representation. 

\paragraph{Evaluation and Privacy:} HealthGAN, ADS-GAN \cite{ehr-12}, CTGAN\cite{ehr-52}, and Pgan \cite{ehr-26} have mechanisms to ensure data privacy, with ADS-GAN emphasizing $\epsilon$-identifiability. The authors of \textbf{HealthGAN}  \cite{ehr-59} introduced an array of metrics to evaluate realism and privacy together called “nearest neighbor adversarial accuracy (AA)”.  \textbf{pGAN} is a privacy preserving GAN that uses these metrics to assess the privacy risk. 


\paragraph{Conditioning:} CTGAN (both  \cite{ehr-50} and \cite{ehr-52} )  are the only models that support conditional generation, indicating their ability to produce data based on certain conditions or labels. \textbf{ADS-GAN} use a modified conditional GAN framework where conditioning variables are not pre-determined but rather optimized from the real patient records, while minimizing patient identifiability. 
% \cite{ehr-12}[ehr-12] \textbf{ADS-GAN} use a modified conditional GAN framework where conditioning variables are not pre-determined but rather optimized from the real patient records, while minimizing patient identifiability. They mathematically define identifiability based on the probability of re-identification given the combination of all data on any individual patient. Later on, \cite{ehr-27}[ehr-27] adapted ADS-GAN for fictitious patient information generation and used a neural network for treatment outcome generation.  They generated synthetic data from a Private Insurance Company in the US dataset, and then demonstrated the use of the generated synthetic data by testing bias in causal effect estimation of four well-established models. 

\paragraph{CTGAN based generation}
Snapshot format data usually have the same properties of tabular data: correlated features, mixed feature type, highly imbalanced categorical features and non-Gaussian distribution of features. These properties impose challenges on the synthetic data generation process. 
CTGANs have been recognized for their effectiveness in generating tabular data, mitigating the challenges and difficulties of this task, and have been adapted to ensure privacy. 
The introduction of DP-CTGAN \cite{ehr-24} offers a deferentially private variant that incorporates random perturbation into the GAN's critic for privacy protection. The federated version, FDP-CTGAN, extends this approach to a distributed data setting, evaluated across multiple medical datasets. 
\cite{ehr-50} use \textbf{CTGANs} for data augmentation purposes (with varying sizes of augmentation) on classification problems. However, the authors of the paper resort to other data balancing methods like SMOTE and ADASYN instead of using the CTGAN for data balancing as well.  The authors of \cite{ehr-47}, on the other hand, use CTGAN as well to address the issue of poor performance of underrepresented sub-populations. They train CTGAN for each sub-population separately and incorporate synthetic samples into the training set of each, consequently increasing the generalizability of predictive models towards underrepresented sub-populations. 
Another paper \cite{ehr-52} utilizes synthetic data generated using CTGAN as a proxy for scarce real-world EHR for the patient length-of-stay multi-class classification task is examined. 





\subsubsection{Diverse papers from diverse formats}

\cite{ehr-70}  later use the \textbf{HealthGAN} to evaluate the fairness properties of generated synthetic data. Previously, synthetic data was evaluated for utility, fidelity, and privacy. This paper extends this and evaluates synthetic data for fairness.  
\cite{ehr-19} implemented \textbf{federated} learning to train separate GANs locally at each organization, and then combining into a central GAN that can generate synthetic discrete EHR, such as ICD-9 codes. \cite{ehr-42} evaluates four different GAN architectures: TGAN, CTGAN, WGAN-GP, and CTABGAN on four tabular medical datasets, three of which are in the snapshot format, and one is an EEG dataset, transformed into a wide flattened tabular dataset. The aim of this study is to study tabular GANs applicability to medical data and analyze whether the GAN architectures specific to tabular data outperform the more general WGAN-GP by evaluating the quality, fidelity, and privacy of the models.
% \cite{ehr-48} apply the \textbf{WGAN-GP} algorithm to generate synthetic one-dimensional medical data (including a radiomics dataset), mainly in the snapshot format, for the purpose of data augmentation. 
% \cite{ehr-53} use \textbf{medGAN} to generate synthetic data from a small dataset from a Low-Middle-Income Countries, and use the synthetic data for training ML models.






